StreamBox-HBM: Stream Analytics on High Bandwidth Hybrid Memory

Stream analytics have an insatiable demand for memory and performance. Emerging hybrid memories combine commodity DDR4 DRAM with 3D-stacked High Bandwidth Memory (HBM) DRAM to meet such demands. However, achieving this promise is challenging because (1) HBM is capacity-limited and (2) HBM boosts performance best for sequential access and high parallelism workloads. At first glance, stream analytics appear a particularly poor match for HBM because they have high capacity demands and data grouping operations, their most demanding computations, use random access. This paper presents the design and implementation of StreamBox-HBM, a stream analytics engine that exploits hybrid memories to achieve scalable high performance. StreamBox-HBM performs data grouping with sequential access sorting algorithms in HBM, in contrast to random access hashing algorithms commonly used in DRAM. StreamBox-HBM solely uses HBM to store Key Pointer Array (KPA) data structures that contain only partial records (keys and pointers to full records) for grouping operations. It dynamically creates and manages prodigious data and pipeline parallelism, choosing when to allocate KPAs in HBM. It dynamically optimizes for both the high bandwidth and limited capacity of HBM, and the limited bandwidth and high capacity of standard DRAM. StreamBox-HBM achieves 110 million records per second and 238 GB/s memory bandwidth while effectively utilizing all 64 cores of Intel's Knights Landing, a commercial server with hybrid memory. It outperforms stream engines with sequential access algorithms without KPAs by 7x and stream engines with random access algorithms by an order of magnitude in throughput. To the best of our knowledge, StreamBox-HBM is the first stream engine optimized for hybrid memories.

==> choice.tex <==
% !TeX root = main.tex

\section{Key Design Choices}
\label{sec:choice}

%\input{fig-arch}

As the top structuring principle, we isolate the engine's data plane from the control plane as well as the underpinning commodity OS, which we deem untrusted in Section~\ref{sec:motiv}. 
As shown in Figure~\ref{fig:arch}, the analytics engine's TCB consists of only the data plane, the trusted execution environment, and the hardware. 
We further minimize the complexity of data plane for shrinking the TCB.
Focusing on the data plane design, we make four design choices.

\begin{myenumerate}
\item \isolation{}
\item \noconcurrency{}
\item \seqmm{}
\item \hints{}
\end{myenumerate}

%\subsection{Enforce the isolation between control plane \& data plane...}
%\subsection{Enforce isolation using hardware}
\subsection{\isolation{}}
\label{sec:choice:isolation}
Our principle of isolating data plane naturally maps to hardware-enforced isolation, such as ARM TrustZone~\cite{arm-trustzone}.  
Widely available on modern ARM cores, TrustZone logically partitions a platform's hardware resources, e.g. DRAM and IO, into a normal (i.e. unsecure) world and a secure world.
%Individual CPU cores can independently switch between two worlds, but only through executing a special \code{SMC} instruction.
CPU cores can independently switch between the two worlds.
%In recent practice, the \sw{} is managed by a trusted OS kernel~\cite{optee,sierra-tee}.
The \sw{} is often managed by a lean, trusted execution environment~\cite{optee,sierra-tee}, which occupies as few as a few hundred KB of memory at run time.
% TEE ram and code size

%For strong isolation, the environment statically partitions the platform resources at boot time.
%, which is capable of running multiple secured software components delegated by different apps.
% offering protection similar to that a commodity OS runs multiple user processes. 
%The API exposed by the trusted OSes are converging to a standard~\cite{globalplatform-tee-guide} in recent years.
%We observe that the interface and structure of trusted OSes are converging to a standard~\cite{globalplatform-tee-guide}.
%The interface and structure of trusted OSes are being standardized in recent years~\cite{globalplatform-tee-guide}.

\TZ{} keeps the entire path of streaming data -- from data arrival at the edge until its departure to the cloud -- in the \se{} and thus shields the path from the untrusted commodity OS.
No extra software effort, e.g. cryptography, is needed for protecting the data. % to protect the data path.

%With isolated environments created by \TZ{}, the entire path of streaming data 
%%-- from input to output, including the IO device drivers -- 
%-- from data arrival at the edge until its departure to the cloud -- 
%remains in the secure world and is thus shielded from the untrusted commodity OS.
%%by design, the data, as it travels across various layers of the hardware/software stack, is able to remain in the secure world.
%No extra software effort, e.g. cryptography, is needed for data protection. % to protect the data path.

However, the \se{}'s physical memory is often limited, challenging data-intensive computation in the data plane.
In \TZ{} practice, a trusted bootloader statically partitions the system DRAM at boot time between two worlds for strong isolation.
To cater to the feature-rich normal world, 
the bootloader often limits the \se{}'s DRAM portion to tens of MB.
This constraint has a strong impact on our memory management design, as will be presented in Section~\ref{sec:mm}.
%Furthermore, some systems, in defending against DRAM bus sniffing attacks,
%restrict the \se{} to only using on-chip SRAM~\cite{sentry} or even CPU cache~\cite{TZ-CaSE}, which are even smaller, at most a few MB.

%\note{a few words on world switch}
%Interrupts often first arrive the secure world, which handles the ones for secure IO and dispatches the remainder to the normal world for handling.
%\note{mention secure memory limit}

\begin{comment}
\paragraph{Protecting multiple apps}
One common criticism against TrustZone is that, due to its limited number of ``worlds'', lacks direct hardware support for multiple applications. 
However, we do not see this as a major limit for supporting IoT edge analytics: 
i) unlike the multi-tenant cloud environment, today's most IoT deployment run one analytics engine owned by one user;
ii) today's trusted OSes governing the secure environment \cite{optee,sierra-tee} are capable of executing secure software components belonging to different applications concurrently, offering isolation similar to a commodity OS, e.g. separate address spaces.
\end{comment}

\paragraph{Alternative approach: Intel SGX}
An alternative to \TZ{} is Intel SGX~\cite{intel-sgx} that allows a user process to create an \textit{enclave} in the process's address space.
%Focusing on isolating CPU execution in the cloud, SGX allows a user process to create a \textit{reverse sandbox}, called enclave, in the process's address space; 
With SGX, the CPU shields the enclave's code and data from the untrusted OS.
%\hp{Exploiting this primitive, sensitive data can be protected being processed~\cite{securestreams}.}
%which are assumed untrusted. 
Unlike TrustZone that partitions the whole platform into two worlds, SGX is CPU-centric: by design, any security-sensitive data sent to/from an enclave has to travel through the untrusted OS, and therefore must be protected by cryptography. 
This is demonstrated in recent work that uses SGX to protect data in stream processing~\cite{securestreams}.
Although recent research proposes to bypass the untrusted OS by relying on a trusted, specialized hypervisor~\cite{sgxio}, 
%by directly bridging the enclave to a low-level trusted layer (e.g. a specialized hypervisor)~\cite{sgxio}, 
we view that SGX offers \textit{indirect} support for protecting streaming data on the edge. 
Therefore, we present our design in the remainder of the paper by assuming the use of TrustZone.

%and is incompatible with analog sources that connect to the edge platform through ADC. 

%In the remainder of this proposal, we will propose research based on the use of ARM TrustZone for brevity.
%For brevity, we will present our proposed research based on TrustZone in the remainder of this proposal.\\

\subsection{\noconcurrency{}}
The data plane should expose low-level abstractions for computations over the protected data. 
The abstraction level should be much lower than the declarative operators that constitute pipelines (\S\ref{sec:motiv:pipeline}). 
Our rationales are as follows.

First, a declarative operator instance, e.g. GroupBy, often deserves parallel execution on multicore. 
If the data plane exposes an interface for executing one entire operator, it would have to embrace its own mechanism for thread management and synchronization.
This often requires sophisticated logic and hence bloats the TCB. 
For instance, an OpenMP library \code{libgomp} has over 40K SLoC~\cite{libgomp}.

Second, although the low-level computation abstractions require the control plane to invoke the data plane more often, the cost of world switch on modern ARM CPUs is as cheap as a few thousand cycles, as reported by prior work~\cite{azab14ccs} and confirmed in our evaluation (\S\ref{sec:eval}).
We noticed that this cost is comparable to SGX enclave invocation reported in recent work~\cite{securestreams}.
%\hp{Compared to the cost of invoking SGX enclave~\cite{securestreams}, the world switch overhead is not significant.} \note{2.35s of 1M function calls}
This cost can be further amortized over many data objects in each batch.
%As parallelism is crucial to stream processing performance (\S\ref{sec:motiv:data}), the data plane should support parallel execution on multicore.
%Yet, it should completely leave out concurrency management to the untrusted control plane.
%First, for minimizing TCB, it is crucial to relieve the data plane of thread management, which often requires sophisticated logic. For instance, an OpenMP library \code{libgomp} has over 40K SLoC. \note{citation?}
%Building it into the data plane not only bloats the TCB but also results in redundant scheduling functionalities between the control/data planes.
%For this reason, although pipelines are programmed with declarative data operators as shown in Figure~\ref{fig:pipeline}, 
%As shown in the code of Figure~\ref{fig:pipeline}, analytics programmers often compose pipelines using high-level, declarative data operators, e.g. GroupBy.
% may have internal parallelism that should be mapped to multiple threads \note{ref}. 
%However, we find it inappropriate for the secure data plane to expose these high-level operators. 
%Therefore, the data plane should  not directly implement declarative data operators that are used in pipeline programming, because
%a single operator may have internal parallelism that demands multithreaded execution. 
%Unfortunately, a declarative data operator may have internal task parallelism that demands multithreaded execution. 
%\note{(e.g. pthread lib has 6K SLoC, a OpenMP library (libgomp) has over 40K SLoC. and the secure kernel support?}. 
%For this reason, were the data plane to expose an interface for executing the entire declarative operators shown in Figure~\ref{fig:pipeline}, the data plane would have to embrace its own thread management. 

%Second, world switch overhead is getting lower and can be amortized effectively. 
%Second, although the low-level \task{} interface requires the control plane to invoke \sys{} more often,
%the cost of world switch can be kept low. 
%The world switch on modern ARM CPUs is as cheap as a few thousand cycles~\cite{azab14ccs}, which can be further amortized over many data objects in a batch. 
%World switch on modern ARM CPUs is getting inexpensive, each only taking at most a few thousand cycles~\cite{azab14ccs}. This is as fast as a dummy syscall. 
%Furthermore, since our proposed engine processes data objects in batches, the cost of one world switch can be amortized over many data objects in a batch. 


%To secure the entire data path on the edge platform, \sys{} further implements data ingress and egress as special primitives.
%In composing a pipeline, the normal environment requests \sys{} to bind ingress and egress to secure IO devices (e.g. sensor or network interface) that are owned by the secure environment; 
%the normal environment, however, is unable to access the data. 



\subsection{\seqmm{}}
%\subsection{Sequential buffers as data plane's primary data structure.}
%To encapsulate stream data and operator state in the secure memory, \sys{} adopts a bold design -- using sequential buffers for all of them. 

We choose contiguous, virtually unbounded buffers as the universal containers for all the streaming data and operator state protected in the \sw{}.
This significantly departs from existing stream processing engines.
%memory abstractions in most stream processing engines. 
As described in Section~\ref{sec:motiv:data}, they often create numerous short-lived memory objects and heavily use hash tables, which poorly suit a secure data plane for two reasons.
First, serving frequent allocation requests with scalable performance requires a sophisticated allocator implementation~\cite{inteltbb,jemalloc} that is likely to bloat the TCB.
Second, the hash table's rationale of trading space for time mismatches the limited capacity of secure memory as mentioned in Section~\ref{sec:choice:isolation}.

Catering to unbounded arrays, we design a custom, lightweight allocator to manage them (\S\ref{sec:mm}). 
We further optimize the secure computation performance for operating on contiguous buffers (\S\ref{sec:opt}). 
%We will present the memory management in detail in Section~\ref{sec:mm}.

%\subsection{Sharing performance hints between two planes.}
\subsection{Taking performance hints from the untrusted}

%Disclosing hints to control plane for performance optimization.
Despite the strong control/data isolation,
we devise a narrow interface for the untrusted control plane to disclose its runtime knowledge, most notably its plan for data consumption, to the data plane.
The hints enable the data plane to generate more compact memory layout and reclaim memory more effectively.
As the hints only affect the data plane's memory placement \textit{policy}, 
they will not weaken the targeted data security. 
Misleading hints may increase the usage of secure memory but will not compromise the protection for the data plane.
We will discuss the hints in detail in Section~\ref{sec:mm}.


==> combine-figs.tex <==
\begin{figure}
    \centering
	    	\includegraphics[width=0.42\textwidth{}]{figs/plot/cmp_kp_rec_cache/kp-rec-cache.pdf}
    \caption{\sys{} outperforms alternative implementations, showing the efficacy of \hbma{} and its management of hybrid memory. Benchmark: TopK Per Key}\label{fig:cmp_full_rec}
    \centering
	    \includegraphics[width=0.49\textwidth{}]{figs/mem_pressure}
    \caption{\sys{} dynamically balances its demands for limited memory resources under varying workloads. 
    Benchmark: TopK Per Key
    }\label{fig:adapt}
\end{figure}

==> conclusions.tex <==
% !TeX root = main.tex
\section{Conclusions}
%To process massive streaming data, edge processing is fascinating in terms of reducing cost and delay in sending raw data to the cloud.
%Generally, the trustworthiness is also regarded as key factor of streaming engine besides its performance.
This paper presents \sys{}, a new stream processing engine at the edge.
The data plane of \sys{} is isolated from its control plane and the underlying OS.
The key contribution of \sys{} is the support for parallel, data-intensive processing in a trusted execution environment.
On an octa core ARM machine, \sys{} processes tens of millions of input events per second while keeping the output delay as tens of milliseconds.
\sys{} offers strong data security guarantees.



% processing, with separating engine's control plane from its data plane.
%The control plane manages thread pool for high parallelism and the data plane supports secure primitives isolated by ARM TrustZone with guarantees for data security.
%The data plane supports secure primitives and is shielded by ARM TrustZone.
%Compared to popular stream processing engines on the same hardware,  \sys{} not only offers strong data confidentiality and integrity, but also increases throughput by 46$\times$.

%To process a bunch of IoT data, edge processing is fascinating pertaining to reducing cost and delay in sending raw data to the cloud.


==> fig-filter.tex <==
% !TeX root = main.tex

\begin{wrapfigure}{R}{0.20\textwidth}
\centering
%\vspace{-30pt}		% use as needed
\includegraphics[width=0.20\textwidth]{./figs/op-filter}
%\vspace{-10pt}		% use as needed
%\caption{Inexpensive IoT devices could help democratize \ib{}. The IoT device: A \$10 Raspberry Pi Zero converted to a wall plug for sensing} 
%\caption{A \$10 IoT device (Raspberry Pi Zero W), packed as a wall plug, are ideal for sensing and controlling tasks in \ib{}s. Photo: raspberrypi.org} 
\caption{Our approaches for bringing commodity IoT devices to } 
%Example in (b)~\cite{smart-power-plugs}}
\label{fig:platform}
%\vspace{-10pt}		% use as needed
\end{wrapfigure}


==> fig-hbma.tex <==
% !TeX root = main.tex

%\begin{figure}[t!]
%\centering
%\includegraphics[width=0.30\textwidth{}]{./figs/hbma} 
%\caption{KPA and record reference counts}
%\label{fig:hbma}
%\end{figure}


\begin{wrapfigure}{R}{0.18\textwidth}
\centering
%\vspace{-30pt}		% use as needed
\includegraphics[width=0.18\textwidth]{./figs/hbma}
%\vspace{-10pt}		% use as needed
%\caption{Inexpensive IoT devices could help democratize \ib{}. The IoT device: A \$10 Raspberry Pi Zero converted to a wall plug for sensing} 
%\caption{KPA and record reference counts}
\caption{KPAs and record bundles. RC=reference count. BID=bundle id}
\label{fig:hbma}
\vspace{-10pt}		% use as needed
\end{wrapfigure}


==> fig-join.tex <==
% !TeX root = main.tex

\begin{wrapfigure}{R}{0.20\textwidth}
\centering
%\vspace{-30pt}		% use as needed
\includegraphics[width=0.20\textwidth]{./figs/op-join}
%\vspace{-10pt}		% use as needed
%\caption{Inexpensive IoT devices could help democratize \ib{}. The IoT device: A \$10 Raspberry Pi Zero converted to a wall plug for sensing} 
%\caption{A \$10 IoT device (Raspberry Pi Zero W), packed as a wall plug, are ideal for sensing and controlling tasks in \ib{}s. Photo: raspberrypi.org} 
\caption{Our approaches for bringing commodity IoT devices to } 
%Example in (b)~\cite{smart-power-plugs}}
\label{fig:op-join}
%\vspace{-10pt}		% use as needed
\end{wrapfigure}


==> fig-pipeline.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/pipeline} 
%\missingfigure[figwidth=6cm]{Kernel support}
%\vspace{-10pt}		% use as needed
\caption{Example execution of streaming computation}
\label{tab:pipeline}
\vspace{-10pt}		% use as needed
\end{figure}


==> fig-placement.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.48\textwidth{}]{./figs/placement} 
%\missingfigure[figwidth=6cm]{Kernel support}
%\vspace{-10pt}		% use as needed
\caption{Passing scheduling knowledge to \hbma{} placement. 
The scheduler and memory demand monitor collaboratively map performance tags to memory types}
\label{fig:placement}
%\vspace{-20pt}		% use as needed
\end{figure}


==> fig-sample-minipage.tex <==
% !TeX root = main.tex

\begin{figure}[!t]

	\begin{minipage}[b]{0.23\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/fair/cpu/cpu}
		        \subcaption{CPU}
		\label{fig:gull}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/fair/dsp/dsp}
		        \subcaption{DSP}
		\label{fig:tiger}
	\end{minipage}	

	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/fair/gpu/gpu}
		        \subcaption{GPU}
		\label{fig:tiger}
	\end{minipage}	
	~
	\begin{minipage}[b]{0.23\textwidth}
	%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
	\includegraphics[width=1\textwidth]{figs/plot/fair/wifi/wifi}
	        \subcaption{WiFi}
	\label{fig:tiger}
	\end{minipage}	
		
	\caption{Throughputs of co-running app instances, before and after one instance (marked with *) enters \psbox{}. 
%	\psbox{} ensures fairness by keeping throughputs of other apps largely unchanged.
	}
%	\vspace{-10pt}		% use as needed
	\label{fig:fair}
\end{figure}

==> fig-sample-single.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
%\includegraphics[width=0.45\textwidth{}]{./figs/benchmarks} 
\missingfigure[figwidth=6cm]{Kernel support}
\vspace{-10pt}		% use as needed
\caption{This is the caption figure}
\label{tab:benchmarks}
\vspace{-20pt}		% use as needed
\end{figure}


==> fig-wrapfig.tex <==
% !TeX root = main.tex

\begin{wrapfigure}{R}{0.42\textwidth}
\centering
\vspace{-30pt}		% use as needed
\includegraphics[width=0.40\textwidth]{./figs/arch}
\vspace{-10pt}		% use as needed
%\caption{Inexpensive IoT devices could help democratize \ib{}. The IoT device: A \$10 Raspberry Pi Zero converted to a wall plug for sensing} 
%\caption{A \$10 IoT device (Raspberry Pi Zero W), packed as a wall plug, are ideal for sensing and controlling tasks in \ib{}s. Photo: raspberrypi.org} 
\caption{Our approaches for bringing commodity IoT devices to \ib{}s} 
%Example in (b)~\cite{smart-power-plugs}}
\label{fig:platform}
\vspace{-10pt}		% use as needed
\end{wrapfigure}


==> figs/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> mm-phys.tex <==
% !TeX root = main.tex

\subsection{Managing Physical Pages}
\label{sec:mm:phys}
%Streaming buffers eases physical memory management. 
%Since streaming buffers facilitate data production/consumption in batches, 
%The abstractions of \ubuf{} and \bufgroup{} greatly simplify physical memory management and thus keep TCB small. 
%Since memory is allocated in the unit of \ubuf{}, 
To support the transparent growth of \ubuf{}s, 
the memory allocator manages the underlying physical pages with a simple thread-caching approach~\cite{tcmalloc-www}.
It uses a global pool to organize all the available secure pages in large grains, e.g. 16MB; it uses a set of per-core pools to track the pages allocated from the global pool in smaller grains, e.g. 2MB.
When the allocator needs new physical pages for an \ubuf{}, it will attempt to reclaim pages first from the same \bufgroup{}, then from the local pool, and finally from the global pool.
As the allocator uses a bitmap to track the free/used states of 2MB blocks, finding a free block is as cheap as a few \code{clz} instructions.
%it i) first attempts to reclaim pages from the start of the same \bufgroup{}; 
%ii) if no enough memory is reclaimed, it attempts to allocate from the local pool;
%iii) if no enough memory, it attempts to allocate from the global pool or press other cores to free memory. 
%\note{We will provide rationales of parameter choices in Section XXX.
%We will test granularities and growing strategies...}
%All the secure physical memory available to pipeline execution is divided into same-size large chunks, e.g. 2MB. 
%page table

% Physical mem
%We shrink the size of physical memory exposed to normal world and dedicate it to secure world, which can be mapped to every \ubuf{} on demand.
%The secure memory is split into fixed-size grains, e.g. 2MB.
%We use a bitmap packed in 32 bit integers to track physical memory usage.
%In this way, only one instruction is needed to check availability of every 32 chunks.
%And whenever there is an available 2MB memory region, we use gcc's builtin function clz to determine the offset, which only introduces one more instruction.
%By using bitmap representation, we are able to keep the searching overhead on a negligible level.

==> motiv.tex <==
% !TeX root = main.tex

\section{Background \& Motivation}
\label{sec:motiv}

Describe the architectural characteristics of HBM....

We next briefly introduce the programming and execution models for stream processing, describe existing processing systems and their inadequacies, and present our design objectives. 

\subsection{Stream processing model}
\label{sec:motiv:data}


\subsection{HBM}
For HPC workloads, we understand that...


\subsection{Knights Landing}

a large number of cores. 

each core is relatively simple. Although out of order, 

==> recycle/recycle-bkgnd-exp.tex <==

\subsection{Motivational experiments}
%\begin{itemize}

\begin{figure}[t!]
\centering
\includegraphics[width=0.50\textwidth]{./figs/kp_vs_record.pdf}
\caption{Extract sort expand <k,p> vs. Sort full Records}
%\vspace{-10pt}		% use as needed
\label{fig:kp_vs_record}
\end{figure}

\paragraph{Why HBM array?} 
%What the overhead of extract, copy, duplicate? Show benchmarks of sorting various columns. HMW array is better than operating all columns.
To let ''Hot computations" benefit the high bandwidth of HBM, \sys{} creates HBM array for them by duplicating the column that upcoming operator will work on and by building the indices that point to full records in DRAM. 
Streaming records usually include tens or even more columns, while HMB array only has a few / two needed columns that upcoming operator will consume, so the overhead of processing HBM array is lower than processing full records in terms of memory movement. 
However, creating HMB array has extra overhead: 1) copying target columns from DRAM to HBM; 2) building indices for records in DRAM; 3) shuffling records or dereferencing indices after processing the HBM array. So there is a tradeoff between building HBM array and processing full records. 

To understand the tradeoff, we use Sort, one of ''Hot Computation", as our benchmark. There are two ways to sort a sequence of records: 1) HBM array based Sort, which builds HBM array for records, sort HMB array, and shuffle original records according sorted HMB array; 2) sorting full records directly. In our benchmark, we vary the number of columns in records to compare the performance of these two ways. As the result is shown in Figure~\ref{fig:operators}, the HBM array based Sort is always faster than sorting full records if the number of columns is larger than two.  

What's more, it is not practical to put full records on HBM because of the small capacity of HBM. Our HMB array only extracted one/ few columns from full records, which usually have tens of columns, so it naturelly address the capacity issue of HBM.

So our HBM array mechanism is able to achieve better performance by than processing full records, meanwhile it addresses the capacity issue of HBM. 








==> recycle/recycle-bkgnd.tex <==
\Paragraph{Stream pipeline}
Stream operators are computations to process streaming Records, such as Filter, GroupBy, and others listed in Figure~\ref{fig:operators}. Many operators form a directed graph, which is called Pipeline. A stream engine ingests unbounded streaming Records, performs a network of operators in a pipeline to process these records, and externalizes the final results.   

\note{highlight streaming data arrangement vs. consumption} -- using a running example?


\Paragraph{Windowing}
The most common way to process unbounded streaming data is to window the data into windows based on Records' timestamps. \sys{} supports two types of common windows: Fixed window and Sliding window. Fixed windows slice up time into segments with a fixed size of temporal length; Sliding windows have fixed size as well, but will slide a fixed period every time, which means there are data overlaps between two contiguous windows. 



==> recycle/recycle-compact.tex <==

\note{Compact selected records after Filtering for locality(cut this part...)} 
We keep full records in DRAM. After filtering, many records are logically dead, although they still physically exist. On one hand, selected records sparsely distribute in DRAM, which causes poor cache locality in later accesses; on the other hand, a large amount of filtered useless records still stay in DRAM, which stresses memory capacity pressure. 
Therefore, it make sense to compact selected records to increase cache locality for later accesses and free the memory occupied by unselected records to release the memory pressure.  

However, compacting selected records brings extra overhead of memory movement and invalidates the existing map between records and pointers in HBM array because of the records rearrangement. Moving memoryand rebuilding pointers will increase the whole pipeline's latency since they take CPU cycles. 
To address this challenge, we propose a mechanism called "Asynchronous Compacting", which copies selected records and rebuilds HMB array in background while keeps the original records and pointers to serve queries' accesses, then switch accesses to rearranged records and rebuilt pointers after copying memory and rebuilding pointers are done\note{ref?}.   
Compacting selected records performs random reads and sequential writes. We use hyperthreads to do this asynchronously in background, and the reasons are: 1) random reads can be speedup linearly by using multiple hyperthreads according \note{ref?} and the results of our microbenchmark; 2) hyperthreads won't affect the main thread on the same physical core, which is running more urgent operators, since the random reads that hyperthreads perform are latency bound \note{evidence??}. In order to further optimize the compacting, we use Gather instruction in each hyperthread, which can speed up random reads by 5x according to microbenchmark. After compacting, rebuilding pointers is much easier because selected records are organized in sequential memory space and pointers of records can be easily computed. 
By doing so, our "Asynchronous Compact" is able to bring better cache locality for later accesses on selected records and release memory pressure without introducing performance penalties. \note{figure to show main thread and hyperthread?}



==> recycle/recycle-deref-SMT.tex <==

\paragraph{Challenge} However, HBM array <K,P> are shuffled by GroupByKey and Ps point to all records in a Window that distribute sparsely in DRAM, so the Dereference performs totally random access. While Dereference is in the critical path of a pipeline as well, so the challenge is to optimize those random access in Dereference to improve performance. 

\paragraph{Solution} Inspired by related work ~\cite{li17sc,yang2016elfen}, we address this challenge by using multiple hyperthreads to do Dereference in parallel \note{WRONG !!!}. In order to further optimize the random access, we use gather instructions to load data from those random addresses in each hyperthread. According to our microbenchmark, the Dereference can be speedup almost linearly by hyperthreads and 5x by gather instructions separately. (see more details about hyperthreads and main thread later)


==> recycle/recycle-intro-v1.tex <==
% !TeX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% xzl: This is the Intro. It can be produced as part of the paper PDF and a standalone html.
% -- Don't put any non standard latex commands here. No need to save space.
% 
% html: see summary/
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\isolation}{Enforcing isolation with ARM TrustZone}
%\newcommand{\noconcurrency}{Stay oblivious to concurrency management}
\newcommand{\noconcurrency}{Exposing low-level abstractions of trusted computations}
%\newcommand{\seqmm}{Unbounded arrays as the primary data structure}
\newcommand{\seqmm}{Unbounded arrays as the universal memory abstraction}
\newcommand{\hints}{Exploiting performance hints from the untrusted}

\section{Introduction}
\label{sec:intro}

% --- stream analytics bkgnd ---- %

Stream processing is a key paradigm of modern data analytics. 
A stream processing engine ingests a large number of timestamped data records, 
pushed them (organized in batches) through a pipeline of operators, and produces results. 
Each operator executes continuous computations in the scopes of record time, and may maintain its internal state. 
The rise of IoT challenges stream processing engines with high input throughput (tens of million records per second)~\cite{trill,streambox,spark-streaming} and low output delay (often milliseconds)~\cite{drizzle,streambox}

In stream analytics, the data is flowing while the queries are standing; this contrasts to classic DBMS, where data is standing and queries are flowing. 
Therefore, a unique aspect of stream analytics is that the \spe{} spends most of time \reorging{} streaming data (e.g. grouping by temporal windows or keys). 
The required data move is intensive and heavily stresses memory hierarchy. 
By contrast, quickly consuming the data once it is organized ....
%The entailed data move is intense, and heavily stresses memory hierarchy. 
, actual \textit{consumption} of the data is often as light as scanning (e.g. to aggregate the data).
%Notably, as streaming computations run in the scopes of record time and keys, 
%spends most of its time on \textit{organizing} streaming data (e.g. by temporal windows or keys), much more than consuming the data. 

%A defining feature of stream processing is that it spends most of the time on data \textit{reorganization} (including record windowing, partitioning, and keying), much more than data \textit{consumption}. 
%This is because streaming computation is often on the scopes of temporal windows and keys, in multiple rounds, while the latter often collapses stream state in one pass. 
%The intensive data move heavily stresses modern memory hierarchy. 
%A fundamental challenge posed by large stream processing is high data velocity, which entails massive data move across memory layers.


Modern high-bandwidth memory (HBM), which excels at sequential data move, promise opportunities. 
%comes to rescue. 
%Multiple recent memory technologies introduce into existing memory architecture. 
%From the CPU's perspective, 
%Compared to traditional DRAM, 
Compared to the DRAM, 
\note{check these numbers}
HBM provides 10$\times$ higher bandwidth (hundreds of GB/sec) at 10$\times$ smaller capacity (a few dozen GB). 
%HBM's bandwidth is higher by one order of magnitude (hundreds of GB/sec) while its capacity is lower by one order of magnitude (a few dozen GB). 
%HBM's latency is similar to or slightly higher than that of DRAM. 
%HBM has 5$\times$ higher bandwidth (hundreds of GB/sec) as compared to DRAM (tens of GB/sec), 
%smaller capacity (a few dozen GB), and similar or slightly higher access latency. 
Recent hardware platforms integrate both types of memory, \note{cite}
%Such a heterogeneous memory system often consists of both HBM and DRAM. 
and accordingly provision with rich hardware parallelism at all levels including manycore, hyperthreading, and wide SIMD lanes. 
Such hardware platforms already show strong competence on HPC workloads~\cite{li17sc} and machine learning~\cite{you17sc}.

It
\note{highlight HBM/DRAM differs from DRAM/NVM and poses unique challenges}

\note{highlight the two fundamental design questions: 
benefit stream analytics with HBM; 
manage two complementary, constrained resources for stream analytics}

While such platforms -- with hybrid memory and rich parallelism -- show high promise on stream analytics, existing \spe{}s are incapable of utilizing the hardware for the following reasons:
%few \spe{}s can leverage such high memory bandwidth. 
%They inherently mismatch HBM/DRAM for the following reasons. 


\begin{itemize}
\item 
First, these engines' choices of operator algorithms and data structures (e.g. hashing) heavily rely on random memory access and cannot generate sufficient demand for memory bandwidth. % which mismatches HBM. 
As we will show in Section~\ref{sec:bkgnd}, these engines severely under-utilize HBM bandwidth (only use less than XX\%), 


%\item 
%%Second, they lack data placement strategies that match data size and access patterns with memory characteristics. 
%Second, they lack data placement strategies that match data objects with different memory characteristics. 
%App-oblivious data placement, e.g. managing HBM as a transparent last-level cache, wastes memory bandwidths and hurts performance, as we will show in the paper. \note{need evidence}.

\item
Second, they are unaware of 
%reconcile and therefore operate under
%exploit high memory bandwidth 
two primary memory constraints -- the limited capacity of HBM and the limited bandwidth of DRAM, and therefore 
could not operate under the constraints accordingly. 

\item
Furthermore, they are unaware of the parallelism cap imposed by the DRAM bandwidth, which may waste CPU cores. 
%failed to acknowledge the parallelism cap imposed by the DRAM bandwidth. 

%of different memory types.
%consider the memory bandwidth limit on thread parallelism.

\end{itemize}

%Cache mode: HMB's bandwidth utilization is limited by the relatively slow bandwidth of DRAM; Flat mode: HMB is a NUMA node, which shares the homogeneous address space with DRAM, so existing Non-HBM-aware systems cannot benefit from HBM.



\begin{comment}
%we set to design a \spe{} with three renovated aspects: its operator algorithms, its data organization, and its task scheduling. 
%Our two observations drive the design:
Our design is driven by the following observations on workloads and hardware, respectively: 
\begin{itemize}
\item Stream processing spends much more time on data reorganization (including record windowing, partitioning, and keying) than data consumption. 
This is because the former involve intensive data move in multiple rounds while the latter often collapses the data in one pass. 
\item HBM excels at massively sequential data move. Random memory access cannot create high enough parallelism to exercise the ample bandwidth. 
%\item Only data with high reuse is worth being brought into HBM
%\item HBM benefits performance only when parallelism is high enough
\end{itemize}
\end{comment}

%The key principle of \sys{} is to structure all computations so that expensive ones always perform sequential access over HBM while inexpensive ones may perform random access in DRAM.     
%The key principle of \sys{} is that, through structuring streaming computations and their memory access, high-complexity computations always perform sequential access over HBM, while low-complexity ones may perform random access in DRAM. 

%To suit stream processing to a heterogeneous memory of HBM and DRAM, 

%it ensures computations with high data reuse to always perform sequential access that favors HBM, 
%while allowing computations with low data reuse to perform random access over DRAM. 
%it ensures high-complexity computations to always perform sequential access that well suits HBM, 
%while allowing low-complexity computations to perform random access over DRAM. 
%it \reorg{}s streaming data by always performing sequential memory access (which benefits from ample memory bandwidth);
%it consumes data with random memory access. 

%\paragraph{Structuring computations with distinctive memory reuse patterns}
%Observing that HBM favors sequential, predictable access, \sys{} organizes all the streaming records and operator state in sequential memory layout (called record bundles), in lieu of random-access data structures.  

%\paragraph{Restructuring streaming computations}
%which centers on the following principle: 
To address the two inadequacies, 
Our response is a \spe{} called \sys{}. 
\sys{} centers on two ideas: 
i) To accelerate stream analytics with HBM, 
\sys{} makes data arrangement perform sequential access over HBM (capacity permitting); 
it makes data consumption perform random access over DRAM. 
ii) To manage HBM/DRAM, it trades off between their respective constraints dynamically. 

\noindent

%\paragraph{HBM arrays}
%\paragraph{Separate keys/records for HBM/DRAM}
%\paragraph{Lifting arrangement keys to HBM}
\paragraph{Dynamically lifting keys/pointers to HBM}
\sys{} retrofits the idea of key/value separation~\cite{wisckey,alphasort}:
while storing full records in DRAM, it lifts the record pointers and the \reorg{} key to HBM. 
The resultant \hbma{}s are the virtual representations of intermediate data arrangement results. 
They are the only data structures that \sys{} considers for placing on HBM. 

To arrange streaming data in pipeline execution, \sys{}  dynamically creates \hbma{}s and computes over them. 
%it produces and consumes \hbma{}, as well as reloading \hbma{} with the arrangement keys in the forthcoming data \reorg{}.
%For instance, prior to GroupBy, \sys{} lifts pointers and the column of grouping key as the \hbma{}.
For instance, for MergeByKey, \sys{} lifts pointers and the grouping keys, and merges the resultant \hbma{}s. 
%By contrast, to consume old records and produce new ones, \sys{} accesses full records in DRAM. 
By contrast, \sys{} accesses full records in DRAM lazily. 
Through \hbma{}s, \sys{} uses HBM effectively: \sys{} only places in HBM the minimum necessary data -- pointers and keys -- in order to accelerate the most expensive operations -- data \reorg. 

%With \hbma{}s, \sys{} uses HBM to precisely accelerate data \reorg{}, the most expensive operation in streaming analytics; 

% --- access order --- %
%\paragraph{Arrangement as sequential access; Consumption as random access}
\paragraph{Structuring primitives with distinctive access patterns}
Centering on \hbma{}s, 
%\sys{} constructs all its streaming computations with two types of primitives with distinctive memory access patterns. 
\sys{} constructs all its streaming computations with \reorg{} and consumption primitives, which exhibit distinctive memory access patterns. 
i) \reorg{} primitives include parallel execution of sort, merge, and join. 
They always access \hbma{}s in sequential order, the key to exploit high memory bandwidth. 
In devising these primitives, we prioritize sequential access pattern over algorithmic simplicity, and therefore opt out hashing-based algorithms.
%chooses sort over hash, despite sort's higher algorithmic complexity. 
ii) consumption primitives: 
they scan \hbma{}s, dereference the pointers, and access full records in DRAM in random order. 
These primitives eschew bringing record data to HBM: the scan is often fast, for which the benefit would not warrant the move cost. 

%By contrast, \sys{} operates on full records in DRAM lazily -- only for producing new records, emitting final results to users, or garbaging collecting dead records. 
%\sys{} produces full records to DRAM lazily -- only when the pipeline produces new data or emits the final results to users. 


Accordingly, \sys{} places all streaming records and operator state in sequential layout (called bundles), in lieu of random-access data structures. 


%Essentially, one \hbma{} represents a virtual bundle consisting of existing records in DRAM. 

%\hbma{}s are sufficiently powerful to support a wide range of \hotop{}s. 


%from full records in DRAM, \sys{} lifts pointers and columns to form \hbma{}s in HBM for the forthcoming data \reorg{} primitives.
%As such, \hotop{}s, such as sort and merge, operate on virtual bundles in reorganizing streaming data. 
%They do so by manipulating the underneath \hbma{}s.

%and access columns in the corresponding whole records in DRAM. 
%As such, \sys{} reorganizes streaming data by consuming and producing \hbma{}s (the virtual bundles they represent). 

%\sys{} materializes \hbma{}s as concrete bundles lazily -- only when pipeline operators produces new records (with new data) that do not exist in concrete bundles or emits the final results to users. 
%\sys{} always place materialized bundles in DRAM and in row format.

%\sys{} dynamically creates HBM arrays for forthcoming \hotop{}s.
%To allocate \hbma{}s, \sys{} always consider HBM first. 
%\hotop{}s are able to consume as high as a few hundred GB/sec of memory bandwidth. 



\note{mention the use of avx512}

%\paragraph{Reconciling resource constraints in streaming allocations}
\paragraph{Reconciling resource pressures in streaming allocations}
\sys{} must operate under two resource constraints of the targeted hybrid memory: 
HBM's limited capacity and DRAM's limited bandwidth. 
%While HBM is full, 
As HBM fills up, streaming data (\hbma{}) has to spill to DRAM; 
as more cores access DRAM, the DRAM bandwidth saturates and diminishes performance return. 
%extra cores will be wasted and see diminishing performance return. 
To prevent one from becoming the single bottleneck, \sys{} monitors and trades off between both resources. 
It does so with a single knob -- the placement of new \hbma{}s: 
when the HBM capacity runs low, it allocates more \hbma{} on DRAM, shifting the pressure towards the DRAM bandwidth;
%when the pressure on DRAM bandwidth increases, it allocates more \hbma{} on HBM, counterbalancing the  
and vice versa.
Therefore, \sys{} places new \hbma{}s based on such a knob modulated by the engine's needs for individual allocations (e.g. performance impact). 
\sys{} avoids migrating existing \hbma{}s, unlike many prior systems for hybrid memory. \note{cite}

%In particular, when DRAM bandwidth is about to saturate, \sys{} throttles the number of worker threads on DRAM and therefore avoids core waste. 


We have implemented \sys{} on Intel Knights Landing, a 64-core processor with 3D-stacked and normal DRAM. 
\sys{} can be standalone running on one machine; multiple \sys{} instances can run on a cluster. 
By evaluating \sys{} on a set of XXX benchmarks, we show that \sys{} achieves input throughput as high as XXX GB/sec while keeping the latency under XXX ms. 
Compared to popular engines, this throughput is XXX higher. 

To the best of our knowledge, \sys{} is the first \spe{} that works on real heterogeneous memory hardware. 
 
%an auxiliary data structure that the engine create dynamically for an upcoming operator. 
%which accompanies a streaming record batch, is created on-demand, and resides in HBM.

%Our key contributions is able to apply to streaming, batch, offline data analysis, kv store, and even in DB.  

% ----- Hongyu's writing. may be useful ---- %
%Our key contribution is especially much more useful for out-of-order data. For example window\_into():
%-- without <k,p>: it has to shuffle/move all records to their corresponding windows according to ts. 
%-- with <k,p>: it can store data as the order as they arrived without moving them during their whole lifetime, because we have pointers and we only operate on <ts, p>.

\note{highlight this is an analytics engine on real heterogeneous memory hardware}

\note{scope -- single node vs. distributed system?}
highlight XYZ can be standalone on one machine or team up to form a distributed system; that is, each XYZ instance can execute a whole pipeline or a portion of the pipeline. 
In this paper, we focus on mechanisms for boosting single node performance. 

==> recycle/recycle-intro.tex <==
In this architecture, the DRAM serves as a high-capacity data store (as before), while the HBM offers ample (5x) memory bandwidth at a reduced capacity. 
To fully exploit HBM memory, such a memory hierarchy is often provisioned with hardware parallelism at all levels including manycore, hyperthreading, and wide SIMD lanes. 
A variety of recent CPUs have already equipped with HBM, including \note{check the SC paper}.... ~\cite{intel-knl} 

\begin{itemize}
\item DRAM. Large capacity. Low bandwidth. Low latency. 
\item On-package Memory. Ample bandwidth. Limited capacity. Notably high latency (20\%). 
The capacity is often GBs, much larger than last-level cache. It can be used as a new cache level which is fully managed by hardware; it can be managed by software explicitly. 
\end{itemize}

A fundamentally challenge posed by large stream processing is high data velocity, which entails massive data move across the memory hierarchy.
Intuitively, this key bottleneck is naturally addressed by an emerging heterogeneous memory architecture as a combination of normal DRAM and high-bandwidth memory (HBM), e.g. on-package DRAM or XXX.
%that is often stacked atop the processor package.

by contrast, \coldop{}s may dereference indices in HBM and access record columns stored in DRAM in random order. 
 
\note{need a figure}




%\paragraph{Bandwidth-aware scheduling}

%\paragraph{Co-designing scheduling and memory placement}
\paragraph{Coupling memory placement with parallelism}
\sys{} dynamically decides the \hbma{} placement based on the engine parallelism, and vice versa. 
%\sys{} considers the interplay between memory bandwidth and thread parallelism.
First, based our insight 2, it places \hbma{}s on HBM only when the parallelism is sufficiently high, and otherwise on the spacious DRAM. 
Second, 
when the parallelism is high and HBM runs low, \sys{} spills \hbma{}s to DRAM and runs (less urgent) \hotop{}s directly on DRAM. 
In such a case, \sys{}, through its global task scheduler, throttles the number of parallel tasks that work on DRAM, so that DRAM bandwidth is never oversubscribed. 
%when \sys{} has to spill \hbma{}s to DRAM due to HBM capacity limit, \sys{}, through its global task scheduler, throttles the number of parallel tasks that work on DRAM, so that DRAM bandwidth is never oversubscribed. 
%control the parallelism over HBM/DRAM to match their respective bandwidths.
%At its global task scheduler, \sys{} throttles the number of parallel tasks that work on DRAM, so that DRAM bandwidth will not be oversubscribed by worker threads. 

\paragraph{Parallelism throttling}
%In allocating \hbma{}, \sys{} allocates HBM arrays are allocated on the HBM. 
%HBM often has a limited capacity.
When HBM runs short, \sys{} has to allocate \hbma{}s on DRAM. 
In such a case, 
\sys{} executes \hotop{} on two types of memory. 
Based our insight 2, \sys{} must consider memory bandwidth and thread parallelism.
\sys{} throttles thread parallelism by memory types. 
In scheduling \hotop{}s, it tags each computation task by the memory type (HBM or DRAM) that the task works on.
%HBM tasks only operate on HBM; 
%DRAM tasks will operate on DRAM. 
At its global task scheduler, \sys{} caps the number of parallel DRAM tasks so that DRAM bandwidth will not be oversubscribed by excessive worker threads. 
(by contrast, it does not cap the parallel HBM tasks). 
\note{XXX mention scheduling earlier}


% ---- formal desc of hbma ---- %


%All computations operate based on a simple memory abstraction -- \hbma{}.
%For a given record batch $R$, an \hbma{} $A_{R, h}$ is an auxiliary data structure that stores a particular column $h$ of all records in batch $R$ and the logic order among these records. 
%a compact representation (a compact replica) of one column in a record batch.
%a compact, in-HBM replica of one specific column in a record batch.
For a given record batch $R$,
an HBM array $A_{R, h}$ is a sequence of pointer/value pairs (\note{inaccurate}) extracted from $R$;
in each pair, the pointer points to a whole record in batch $R$, while the value is a copy from the column $h$ of this record.
%where the indices point to whole records in the batch, and the keys are replicas from a specific column of the batch (the HBM may contain dirty keys). 
\Hotop{}s always operate on HBM arrays with no need for dereferencing the pointers, e.g. to shuffle pointer/value pairs. 
They perform sequential memory access. 
%They perform sequential memory access that exercises the memory bandwidth. 
%For instance, to merge two record batches, \sys{} builds their respective (key,index) HBM arrays and merges them.
\Coldop{}s, by contrast, iterate over \hbma{}s:
they dereference the stored pointers
%follow the pointers in \hbma{}s, 
and access the corresponding whole records in $R$ in random order. 
%and access columns in the corresponding whole records in DRAM. 
The compact layout of \hbma{}s and their sequential access match bandwidth-rich, capacity-constrained HBM.  \\




\hbma{}'s compactness and sequential access pattern match capacity-constrained, bandwidth-rich HBM.  
They effectively utilize the memory bandwidth in that: 
i) unaccessed record columns always reside in DRAM as part of the whole records, and are never brought to HBM nor touched until materialization;
ii) data consumption does not require moving data from DRAM to HBM, where the benefit does not warrant the move cost. 
%\sys{} dynamically creates HBM arrays as auxiliary data of a record batch, and executes \hotop{} over the HBM arrays. 
%As record batches flow through the operators in a pipeline,\sys{} builds an HBM array of the specific column that an forthcoming \hotop{} will consume.
%hence, the \hotop{} thus consumes the HBM array without touching whole records.




%These operators work on sequential memory layout for both streaming records and operator state, in lieu of random-access data structures.  
%that are commonly used in stream processing engines such as hash tables and trees. 

%As a prerequisite, \sys{} creates compact, sequential memory layout of data, and consume the data with parallel executions of sort, merge, and scan, in lieu of random-access data structures that are commonly used in stream processing engines such as hash tables and trees. 

%The central idea of \sys{} is to structure all streaming computations as two categories and 
%exploit the two memory types respectively. 
%%differentiate their data placement: 

%The central idea of \sys{} is to structure all stream processing state as two categories based on their reuseabiltiy in the upcoming computations, so that: 
%\begin{enumerate}
%\item 
%%Computations perform sequential access in HBM for data that exhibits high reuse 
%Computations perform sequential access in HBM over highly reused data.
%\item 
%%Computations exhibiting low data reuse perform random access of DRAM.
%Computations perform random access in DRAM for data that exhibits low reuse 
%\end{enumerate}

%The central idea of \sys{} is to decompose common streaming operators into two categories of computations, and arrange their memory access accordingly: 

%the streaming computations as two categories and arrange their memory access accordingly:


%The central idea of \sys{} is to split all streaming data as two categories, 
%arranging their layout and the streaming computations accordingly, so that: 
%\begin{enumerate}
%\item 
%\textit{Ephemeral} data that exhibits low reuse is placed in DRAM and is accessed randomly.
%\item 
%?? data that exhibits high reuse is placed in HBM and is accessed sequentially.
%%the computations perform sequential access of them; 
%\end{enumerate}


==> recycle/recycle-kpa-primitives-2.tex <==

We next describe primitives that manipulate \hbma{}s. 
We use $\mathscr{R}$ to denote a record bundle. 
We use $\hbma{}(c)$ to denote a \hbma{} with its resident keys from record column $c$. 

\input{tab-hbma}

%\paragraph{Creation}
\noindent
\textbf{Maintenance primitives} convert between \hbma{}s and record bundles, as well as swapping \hbma{}'s resident key. 
\begin{myitemize}
\item Extract: $\mathscr{R} \rightarrow \hbma(c)$.
\sys{} creates a new \hbma{} from a record bundle (always in DRAM). 
%It does so prior to grouping records in a bundle for which \hbma{} does not exist yet (e.g. the records are just ingested). 
To do so, \sys{} replicates the column $c$ to be resident keys and initializes pointers to the records. 

\item Materialization: $\hbma{}(c) \rightarrow \mathscr{R}$
This primitive emits a bundle of full records according to \hbma{}. 
It does so by scans and dereferences the pointers in a \hbma{}, and accordingly copies the full records to the output buffer in DRAM. 

\item Key swapping: $\hbma(c_1) \rightarrow \hbma(c_2)$
It replaces a \hbma{}'s keys with a nonresident column in full records. 
It scans the \hbma{}, deferences the pointers to locate full records, and then overwrites the resident keys with column $c_2$ from the corresponding full records. 
%by gathering data from the new column of the full records. 
The old keys in the \hbma{} can be simply dropped as long as they are unmodified in place. 
Key swapping incurs random access of full records in DRAM. 
\end{myitemize}

\noindent
\textbf{Grouping primitives} operate on \hbma{}s with sequential memory access to exploit HBM (\S\ref{sec:bkgnd}). 
The core algorithms are sort and merge. They access resident keys, and accordingly move around the key/pointer pairs within or across \hbma{}s. 
%As grouping often dominates stream analytics execution, we optimize sort and merge, as will be presented later. 

\begin{myitemize}
\item Sort: $Sort(\hbma{}(c)) \rightarrow \hbma{}(c)$.
It sorts the \hbma{} by the resident keys. 

\item Merge: $Merge(\hbma_1{}(c),\hbma{}_2(c)) \rightarrow \hbma_3{}(c)$.
The primitive scans two \hbma{}s simultaneously, both already sorted by resident column $c$, and produces a new \hbma{}s sorted by column $c$. 

\item Join: $Join(\hbma_1{}(c),\hbma{}_2(c)) \rightarrow \mathscr{R}$. 
Similar to Merge, this primitive scans two sorted \hbma{}s. 
Upon key match on both inputs, it emits new records by combining two records from both inputs. 

\end{myitemize}

%\paragraph{Reduction}

\noindent
\textbf{Reduction primitives} summarize a given column and produce new records. 
They access full records with mostly random access. 
\begin{myitemize}
\item Keyed:  $Reduce(\hbma(c)) \rightarrow \mathscr{R}$. 
The primitive does per-key reduction based on the keys on column $c$. 
It requires a \hbma{} input with resident keys already sorted by the keys.
The primitive scans the \hbma{} in sequential order. 
It dereferences the pointers in \hbma{}s to consumes nonresident column(s) during scan. 
Take per-key aggregation for example, the primitive keeps track of contiguous key ranges in \hbma{}; for each key range, it coalesces all values in a nonresident column. 

\item Unkeyed: $Reduce(\mathscr{R}_1 | \hbma) \rightarrow \mathscr{R}_2$
The primitive does reduction across all records. 
It directly scans a bundle of full records or a \hbma{}, consumes nonresident column(s), and produces a new record bundle.  
\end{myitemize}

\noindent
\textbf{Selection primitives} $Sel(\mathscr{R} | HBM_1(k)) \rightarrow HBM_2(k)$. 
They create a subset of records. They do so by scanning a record bundle or a \hbma{} and produces a \hbma{} with the survival key/pointer pairs. 

==> recycle/recycle-kpa-primitives.tex <==

\paragraph{Extract}
$\mathscr{R} \rightarrow HBM(k)$
\sys{} creates a new \hbma{} out of a record bundle (always in DRAM). 
%It does so prior to grouping records in a bundle for which \hbma{} does not exist yet (e.g. the records are just ingested). 
To do so, \sys{} replicates the record column to be resident keys and populates the sequence of pointers to the full records. 
%Multiple \hbma{}s can be created out of one record bundle. 

%\paragraph{Grouping: Sort, Merge, and RangePartition}
\paragraph{Grouping: Sort and Merge}
All grouping operators operate on \hbma{}s. 
We implement these operators with two \hbma{} compute kernels -- sort and merge, as their sequential access matches HBM well (\S\ref{sec:bkgnd}). 
Both primitives access resident keys, and accordingly move around the key/pointer pairs within or across \hbma{}s. 
As grouping often dominates stream analytics execution, we optimize sort and merge, as will be presented later. 

\paragraph{Key swapping}
$HBM(k_1) \rightarrow HBM(k_2)$
\sys{} replaces the resident keys in \hbma{} with a nonresident column. 
It scans the \hbma{}, deferences the pointers to locate full records, and then overwrites the \hbma{} keys with the new column data from the corresponding full records. 
%by gathering data from the new column of the full records. 
In this process, the old keys in the \hbma{} can be simply dropped as long as they are unmodified in place. 
Key swapping incurs random access of full records in DRAM. 


\paragraph{In-\hbma{} Reduction}
$Reduce(HBM_1(k)) \rightarrow HBM_2(k)$
Scan the \hbma{} and do reduction on the resident key. 
The output is a new (smaller) \hbma{} with the same resident key. 

%\paragraph{Reduction}
%\paragraph{Indirect Reduction}
\paragraph{Out-of-\hbma{} Reduction}
%\subsection{Reduction and Materialization}
%\subsection{Dereference/Expand}
%a. from full records
%b. from one HBM array to another HBM array. <v,p> to <k,p>
$Reduce(HBM_1(k)) \rightarrow HBM_2(k)$
Reduction on specific value column(s) often follows grouping operators, e.g. per-key aggregation of values. 
%Following a similar procedure of dereferencing the pointers in \hbma{}s and accessing the value column 
%Similar to key swapping, \sys{} dereferences the pointers in \hbma{}s in sequence, accesses the value column, and consumes the values on-the-fly. 
Similar to key swapping, \sys{} scans \hbma{} in sequential order. 
It dereferences the pointers in \hbma{}s to access the value column in full records, and consumes the values on-the-fly. 
For keyed reduction, \sys{} sorts \hbma{} on the resident key prior to indirect reduction. 
In the aggregation example above, \sys{} keeps track of contiguous key ranges in \hbma{}; for each key range, it coalesces all values gathered from the full records. 
As its result, reduction may update columns in the existing records, or produce new records.
\sys{} always place new records in DRAM. 
The reduction generates random access of full records in DRAM. 

\paragraph{Materialization}
$HBM(k) \rightarrow \mathscr{R}$
A pipeline, at its egress, will eventually materialize its output, i.e. emitting bundles of full records according to \hbma{}. 
It does so by scans and dereferences the pointers in a \hbma{}, and accordingly copies the full records to the output buffer in DRAM. 

==> recycle/recycle-output-records.tex <==

Most operators extract one or several columns from existing records in DRAM without outputting new types of record, such as Filtering, Groupby, and SortByKey. However, some other operators, like Join, AveragebyKey, and other aggregators,  will emit new types of records after processing input records. As Figure~\ref{fig:pplexample} shows, the input record type of SumVperK is R<k0, v0, v1...>, while the output record type is R<k0, sumV>. So the problem is where to output new records.  \sys{} addresses this issue by placing new records on HBM and DRAM based on reuse pattern, access pattern, the number of columns of new records, and the memory pressure.

1) Reuse pattern: new records should go to DRAM if they will not be processed any more in the future. For example, the downstream is Sink in Figure~\ref{fig:pplexample} \circled{7}, in which case we store records on DRAM directly. 

2) Records with no more than two columns: we don't extract HBM array for them, since it is same to process two columns of HBW array and two columns of full records. In this case, \sys{} places records according to the access pattern. If downstream operator performs sequential access, then records go to HBM as shown in Figure~\ref{fig:pplexample} \circled{5}; otherwise records go to DRAM as shown in Figure~\ref{fig:pplexample} \circled{7}. 

3) Records with more than two columns: \sys{} places these records on DRAM by default as shown in Figure~\ref{fig:pplexample} \circled{7}. According to our motivational experiment result in Figure~\ref{fig:kp_vs_record}\}, processing HBM array is always faster than processing full records. So \sys{} will extract HBM array from new records based on the column that downstream operator will work on as shown in Figure~\ref{fig:pplexample} \circled{6}, if the downstream operator performs sequential access.

==> recycle/recycle-sort-vs-hash.tex <==
\textit{Predominating sequential access}
Sequential access is known crucial to good memory bandwidth utilization.  \note{cite}
To utilize the memory bandwidth of HBM, the need for sequential access even triumphs over algorithmic simplicity.
%The ample memory bandwidth changes many important, well-known trade offs. 
%The sequential access pattern even triumphs over algorithmic simplicity.
In the microbenchmark above, hashing and sorting are known as duals in implementing GroupBy.
For long, hashing has been a preferred choice -- despite its random memory access, its algorithmic complexity is lower. \note{cite}.
HBM (together with our SIMD-optimized mergesort) has changed this trade-off. 
As shown in figure~\ref{fig:motiv}, 
\sort{} on Knights Landing (Sort/HBM) outperforms \hash{} on Knights Landing (Hash/HBM) by up to XX $\times$.
Sort/HBM even outperforms \hash{} on a high-cost, 56 core Xeon server (Hash/Xeon) by up to XX $\times$. 
%\sort{} on Knights Landing outperforms \hash{} by up to XX $\times$ on the same machine and 
%This performance also exceeds \hash{} running on a high-end Xeon server (Intel Xeon E7-4850v4, 56 cores in total).
Furthermore, \sort{} substantially benefits from HBM: 
when running on DRAM (Sort/DRAM), it is bound by the XXX GB/sec DRAM gibandwidth and fails to scale beyond 16 cores.
By contrast, \hash{} sees little throughput difference when running on HBM (Hash/HBM) or DRAM (Hash/DRAM).
%By contrast, \hash{} even sees slight throughput decrease when running on HBM (Hash/HBM) as compared to running on DRAM (Hash/DRAM).
%a slight throughput drop on due to higher memory latency. 
Under the hood, \sort{} utilizes more than 250GB/sec of memory bandwidth, while \hash{} utilizes less than XXXGB/sec.
\textbf{Our observation should not be read as report of absolute performance of hash on KNL, but as advocate for sequential memory access. 
Besides, we notice hand-vectorized and optimized hash for KNL also reports low HBM utilization.}

==> tab-hbma.tex <==
% !TeX root = main.tex

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
%\footnotesize
\centering
%\caption{Definitions}
\caption{Terminology}
\label{tab:definitions}
\vspace*{-1em}
\begin{tabular}{|c|l|l|l|l|}
\hline
\multirow{3}{*}{Maintenance} & Extract  &  $\mathscr{R} \rightarrow HBM(k)$ & 
\sys{} creates a new \hbma{} out of a record bundle (always in DRAM). To do so, \sys{} replicates the record column to be resident keys and populates the sequence of pointers to the full records. 
 &  \\ \cline{2-5} 
                    & Key swap &  &  &  \\ \cline{2-5} 
                    & Materialization &  &  &  \\ \hline
\multirow{2}{*}{Grouping} & Sort &  &  &  \\ \cline{2-5} 
                    & Merge &  &  &  \\ \hline
\multirow{3}{*}{Reduction} & In-KPA &  &  &  \\ \cline{2-5} 
					& Out-of-KPA &  &  &  \\ \cline{2-5} 
                    & Join &  &  &  \\ \hline                    
\end{tabular}
\vspace*{-2em}
\end{table*}


==> tab-primitives.tex <==
% !TeX root = main.tex

\begin{table}[]
\centering
	\vspace{1pt}
    \includegraphics[width=0.46\textwidth]{figs/operators}
    \caption{Important \task{}s (columns) and declarative operators (rows) they constitute. 
    The current \sys{} implementation includes 27 \task{}s in total }
	\label{tab:operators}
\end{table}



==> tab-sample-2col.tex <==
% !TeX root = main.tex

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
%\footnotesize
\centering
%\caption{Definitions}
\caption{Terminology}
\label{tab:definitions}
\vspace*{-1em}
 \begin{tabular}{|c|l|r|r|r|r|}
 \hline
 & \multicolumn{1}{c|}{Text} & \multicolumn{1}{c|}{Text} & \multicolumn{1}{c|}{Text} & \multicolumn{1}{c|}{Text} & \multicolumn{1}{c|}{text}\\
 \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Maint.}}} & Extract & $\mathscr{R} \rightarrow HBM(k)$ & Creates a new \hbma{} out of a record bundle. To do so, \sys{} replicates the record column to be resident keys and populates the sequence of pointers to the full records. &&\\
 & Materialization & $HBM(k) \rightarrow \mathscr{R}$ &&&\\
 & Key swapping & $HBM(k_1) \rightarrow HBM(k_2)$ & &&\\
 \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Group}}} & text &&&&\\
 & text &&&&\\
 & text &&&&\\
 \hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Reduce}}} & In-\hbma{} & $Reduce(HBM_1(k)) \rightarrow HBM_2(k)$ &&&\\
 & Out-of-\hbma{} &&&&\\
 & Join &&&&\\
 \hline  
 \end{tabular}
\vspace*{-2em}
\end{table*}


==> tab-sample-latex.tex <==
% !TeX root = main.tex

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\footnotesize
\centering
%\caption{Definitions}
\caption{Terminology}
\label{tab:definitions}
\vspace*{-1em}
\begin{tabular}{@{}l@{$\;\;$}p{2.65in}@{}}
% 	\rowcolor[HTML]{000000} 
% {\color[HTML]{FFFFFF} \textsf{term}} & {\color[HTML]{FFFFFF} \textsf{explanation}}                                               \\
%\textsf{\textbf{term}} &
%\textsf{\textbf{definition}} \\ \toprule
\toprule[0.7pt]%\midrule[0.3pt]

\textsf{\textrm{Term}} &
\textsf{\textrm{Definition}} \\ \toprule
	Stream                                               & An
        unbounded sequence of records              \\
	Transform                                         & A computation that consumes and produces streams         \\
	Pipeline                                             & A dataflow graph of transforms                                                   \\
	Watermark                                         & A
        special event timestamp for marking stream progression \\
	Epoch                                                & A set of  records arriving between two watermarks                           \\
	Bundle & A set of records in an epoch (processing unit of work) \\
	Evaluator & A worker thread that processes bundles and watermarks \\
	Container                                            &
        Data structure that tracks watermarks, epochs, and bundles\\
%	Window & A temporal processing scope of one or more epochs \\
	Window & A temporal processing scope of records \\
\midrule[0.7pt]
%\midrule[0.3pt]\bottomrule[1pt]
\end{tabular}
\vspace*{-2em}
\end{table}

